Learning the CSI Denoising and Feedback Without Supervision

In this work, we develop a joint denoising and feedback strategy for channel state information in frequency division duplex systems. In such systems, the biggest challenge is the overhead incurred when the mobile terminal has to send the downlink channel state information or corresponding partial information to the base station, where the complete estimates can subsequently be restored. To this end, we propose a novel learning-based framework for denoising and compression of channel estimates. Unlike existing studies, we extend a recently proposed approach and show that based solely on noisy uplink data available at the base station, it is possible to learn an autoencoder neural network that generalizes to downlink data. Subsequently, half of the autoencoder can be offloaded to the mobile terminals to generate channel feedback there as efficiently as possible, without any training effort at the terminals or corresponding transfer of training data. Numerical simulations demonstrate the excellent performance of the proposed method.

==> new_plots/bar_plot2.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
% \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\definecolor{color0}{HTML}{CA6F1E}
\definecolor{color1}{HTML}{7FB3D5}


\begin{axis}[
axis line style={white!15!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=none},
tick align=outside,
tick pos=left,
x grid style={white!80!black},
xmin=-0.2925, xmax=2.2925,
xtick style={color=white!15!black},
xtick={0,1,2},
xticklabels={ENC,DEC,AE},
y grid style={white!80!black},
ylabel={$\#$ Parameters},
ymin=0, ymax=4416463.8,
ytick style={color=white!15!black}
]
\draw[draw,fill=color0] (axis cs:-0.175,0) rectangle (axis cs:-0.025,426744);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{AE}

\draw[draw,fill=color0] (axis cs:0.825,0) rectangle (axis cs:0.975,575226);
\draw[draw,fill=color0] (axis cs:1.825,0) rectangle (axis cs:1.975,1001970);
\draw[draw,fill=color1] (axis cs:0.025,0) rectangle (axis cs:0.175,2097450);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1};
\addlegendentry{CsiNet}

\draw[draw,fill=color1] (axis cs:1.025,0) rectangle (axis cs:1.175,2108706);
\draw[draw,fill=color1] (axis cs:2.025,0) rectangle (axis cs:2.175,4206156);
\end{axis}

\end{tikzpicture}


==> plots_10db/bar_plot.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{HTML}{CA6F1E}

\begin{axis}[
axis line style={white!15!black},
tick align=outside,
tick pos=left,
x grid style={white!80!black},
xmin=-0.315, xmax=3.315,
xtick style={color=white!15!black},
xticklabels={{}, DEN, {}, ENC, {}, DEC, {}, AE},
y grid style={white!80!black},
ymin=0, ymax=1052068.5,
ytick style={color=white!15!black}
]
\draw[draw,fill=color0] (axis cs:-0.12,0) rectangle (axis cs:0.12,72514);
\draw[draw,fill=color0] (axis cs:0.88,0) rectangle (axis cs:1.12,426744);
\draw[draw,fill=color0] (axis cs:1.88,0) rectangle (axis cs:2.12,575226);
\draw[draw,fill=color0] (axis cs:2.88,0) rectangle (axis cs:3.12,1001970);
\end{axis}

\end{tikzpicture}


==> plots_10db/box_plot.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.843137254901961,0.0980392156862745,0.109803921568627}
% \definecolor{color1}{rgb}{0.172549019607843,0.482352941176471,0.713725490196078}
\definecolor{color0}{HTML}{F9E79F}
\definecolor{color1}{HTML}{85C1E9}

\begin{axis}[
axis line style={white!15!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=none},
tick align=outside,
tick pos=left,
x grid style={white!80!black},
xmin=-2, xmax=4,
xtick style={color=white!15!black},
xtick={0,2},
xticklabels={DEN,AE},
y grid style={white!80!black},
ymin=-0.00412610583007336, ymax=0.120158549770713,
ytick style={color=white!15!black},
ytick={-0.02,0,0.02,0.04,0.06,0.08,0.1,0.12,0.14},
yticklabels={−0.02,0.00,0.02,0.04,0.06,0.08,0.10,0.12,0.14}
]

\addlegendimage{area legend, thick,fill = color0}
\addlegendentry{$\varepsilon^2$}

\addlegendimage{area legend, thick,fill = color1}
\addlegendentry{$1-\rho$}

\addplot [black, dotted, forget plot]
table {%
-0.3 0.00935916672460735
-0.3 0.00291019165888429
};
\addplot [black, dotted, forget plot]
table {%
-0.3 0.0164774139411747
-0.3 0.027102155610919
};
\addplot [black, forget plot]
table {%
-0.375 0.00291019165888429
-0.225 0.00291019165888429
};
\addplot [black, forget plot]
table {%
-0.375 0.027102155610919
-0.225 0.027102155610919
};
\addplot [black, dotted, forget plot]
table {%
1.7 0.028373084962368
1.7 0.00473171472549438
};
\addplot [black, dotted, forget plot]
table {%
1.7 0.0628994200378656
1.7 0.114509247243404
};
\addplot [black, forget plot]
table {%
1.625 0.00473171472549438
1.775 0.00473171472549438
};
\addplot [black, forget plot]
table {%
1.625 0.114509247243404
1.775 0.114509247243404
};
\addplot [black, dotted, forget plot]
table {%
0.3 0.00483138859272003
0.3 0.00152319669723511
};
\addplot [black, dotted, forget plot]
table {%
0.3 0.00854584574699402
0.3 0.0141090154647827
};
\addplot [black, forget plot]
table {%
0.225 0.00152319669723511
0.375 0.00152319669723511
};
\addplot [black, forget plot]
table {%
0.225 0.0141090154647827
0.375 0.0141090154647827
};
\addplot [black, dotted, forget plot]
table {%
2.3 0.0149180293083191
2.3 0.00223350524902344
};
\addplot [black, dotted, forget plot]
table {%
2.3 0.0334646552801132
2.3 0.0612514615058899
};
\addplot [black, forget plot]
table {%
2.225 0.00223350524902344
2.375 0.00223350524902344
};
\addplot [black, forget plot]
table {%
2.225 0.0612514615058899
2.375 0.0612514615058899
};
\path [draw=black, fill=color0]
(axis cs:-0.45,0.00935916672460735)
--(axis cs:-0.15,0.00935916672460735)
--(axis cs:-0.15,0.0164774139411747)
--(axis cs:-0.45,0.0164774139411747)
--(axis cs:-0.45,0.00935916672460735)
--cycle;
\path [draw=black, fill=color0]
(axis cs:1.55,0.028373084962368)
--(axis cs:1.85,0.028373084962368)
--(axis cs:1.85,0.0628994200378656)
--(axis cs:1.55,0.0628994200378656)
--(axis cs:1.55,0.028373084962368)
--cycle;
\path [draw=black, fill=color1]
(axis cs:0.15,0.00483138859272003)
--(axis cs:0.45,0.00483138859272003)
--(axis cs:0.45,0.00854584574699402)
--(axis cs:0.15,0.00854584574699402)
--(axis cs:0.15,0.00483138859272003)
--cycle;
\path [draw=black, fill=color1]
(axis cs:2.15,0.0149180293083191)
--(axis cs:2.45,0.0149180293083191)
--(axis cs:2.45,0.0334646552801132)
--(axis cs:2.15,0.0334646552801132)
--(axis cs:2.15,0.0149180293083191)
--cycle;
\addplot [black, forget plot]
table {%
-0.45 0.0122349499724805
-0.15 0.0122349499724805
};
\addplot [black, forget plot]
table {%
1.55 0.0394142158329487
1.85 0.0394142158329487
};
\addplot [black, forget plot]
table {%
0.15 0.00634670257568359
0.45 0.00634670257568359
};
\addplot [black, forget plot]
table {%
2.15 0.0208609700202942
2.45 0.0208609700202942
};
\end{axis}

\end{tikzpicture}


==> plots_10db/lisa_plot.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}
\definecolor{color0}{rgb}{0.843137254901961,0.0980392156862745,0.109803921568627}
\definecolor{color1}{rgb}{0.172549019607843,0.482352941176471,0.713725490196078}


\begin{axis}[
axis line style={white!15!black},
legend cell align={left},
legend style={nodes={scale=0.84, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.0,1.0)}, anchor=north west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!80!black},
xlabel={SNR [dB] = Average TX power},
xmajorgrids,
xmin=-12, xmax=32,
xtick style={color=white!15!black},
xtick={-15,-10,-5,0,5,10,15,20,25,30,35},
xticklabels={\(\displaystyle -15\),\(\displaystyle -10\),\(\displaystyle -5\),\(\displaystyle 0\),\(\displaystyle 5\),\(\displaystyle 10\),\(\displaystyle 15\),\(\displaystyle 20\),\(\displaystyle 25\),\(\displaystyle 30\),\(\displaystyle 35\)},
y grid style={white!80!black},
ylabel={Per-user Rate [bpcu]},
ymajorgrids,
ymin=-0.322982006232411, ymax=7.76019947743808,
ytick style={color=white!15!black},
ytick={0, 1, 2, 3, 4, 5, 6, 7},
yticklabels={\(\displaystyle 0\),\(\displaystyle 1\),\(\displaystyle 2\),\(\displaystyle 3\),\(\displaystyle 4\),\(\displaystyle 5\),\(\displaystyle 6\),\(\displaystyle 7\)},
]
\addplot [line width =1pt, color0]
table {%
-10 0.0512375247634074
-5 0.13415986490384
0 0.319906061481726
5 0.704004076241574
10 1.42220603975875
15 2.5601456191306
20 4.00443827915319
25 5.58927877107164
30 7.22528081553312
};
\addlegendentry{Perfect CSI, $\Delta f = 120$~MHz}
\addplot [line width =1pt, color0, dashed]
table {%
-10 0.0464618609917164
-5 0.122640264384841
0 0.294128211158616
5 0.650186747450236
10 1.31751665316361
15 2.37991753180541
20 3.71357190012226
25 5.08609175512106
30 6.2988889442369
};
\addlegendentry{AE, $\Delta f = 120$~MHz}
\addplot [line width =1pt, color0, dotted]
table {%
-10 0.0444353339344291
-5 0.117062337092519
0 0.277696754803346
5 0.599263128271472
10 1.15504198550918
15 1.92412896881133
20 2.71261766097414
25 3.33383057972393
30 3.74153874680032
};
\addlegendentry{IDFT, $\Delta f = 120$~MHz}
\addplot [line width =1pt, color1]
table {%
-10 0.0566815775385364
-5 0.146576907538984
0 0.347404598977262
5 0.7583089024838
10 1.51781700591805
15 2.69566152167743
20 4.16104749644407
25 5.7540245565629
30 7.39278213727124
};
\addlegendentry{Perfect CSI, $\Delta f = 480$~MHz}
\addplot [line width =1pt, color1, dashed]
table {%
-10 0.0515669519027448
-5 0.134280739910432
0 0.319730075363717
5 0.700101961158818
10 1.40525782280892
15 2.50598876966379
20 3.85565766922824
25 5.22091314356586
30 6.40690242325547
};
\addlegendentry{AE, $\Delta f = 480$~MHz}
\addplot [line width =1pt, color1, dotted]
table {%
-10 0.0491876691875123
-5 0.128573132419412
0 0.303455226497199
5 0.64966121636637
10 1.24510268029969
15 2.06118462085636
20 2.89080034574552
25 3.54517794539324
30 3.97666820523595
};
\addlegendentry{IDFT, $\Delta f = 480$~MHz}
\end{axis}

\end{tikzpicture}

